Universal Multi-modal Entity Alignment via Iteratively Fusing Modality Similarity Paths

The objective of Entity Alignment (EA) is to identify equivalent entity pairs from multiple Knowledge Graphs (KGs) and create a more comprehensive and unified KG. The majority of EA methods have primarily focused on the structural modality of KGs, lacking exploration of multi-modal information. A few multi-modal EA methods have made good attempts in this field. Still, they have two shortcomings: (1) inconsistent and inefficient modality modeling that designs complex and distinct models for each modality; (2) ineffective modality fusion due to the heterogeneous nature of modalities in EA. To tackle these challenges, we propose PathFusion, consisting of two main components: (1) MSP, a unified modeling approach that simplifies the alignment process by constructing paths connecting entities and modality nodes to represent multiple modalities; (2) IRF, an iterative fusion method that effectively combines information from different modalities using the path as an information carrier. Experimental results on real-world datasets demonstrate the superiority of PathFusion over state-of-the-art methods, with 22.4%-28.9% absolute improvement on Hits@1, and 0.194-0.245 absolute improvement on MRR.

==> src/algorithms/pseudo_code.tex <==

\begin{algorithm}[!t] \small
	%\SetAlgoNoLine %控制有无竖线
	\caption{\Method{} process} 
     \label{alg:pseudo_code}
	\KwIn{KGs $G_s, G_t$ with collection of modalities $\mathcal{X}$, seed alignment $\phi^{\prime}$}
	\KwOut{Alignment matrix $M$}
    \textcolor{blue}{/* Step 1: train relational encoder by  $\phi^{\prime}$ and derive mapping matrix $M_X$ for each modality by \Path{} */}\\
    $\boldsymbol{H}_s, \boldsymbol{H}_t \leftarrow$ Relational-Encoder $\left(G_s, G_t, \phi^{\prime}\right)$\\
	\For{$X \in \mathcal{X}$} 
	{ 
        $M_X \leftarrow$ \Path{} (X) \\
	}
    \textcolor{blue}{/* Step 2: Iteratively fuse information from different modalities by \Fuse{} */}\\
    \For{$e \in range(3)$}
    {
        $M \leftarrow \operatorname{Sinkhorn}(\boldsymbol{H}_s\left(\boldsymbol{H}_t\right)^T + \sum_{X \in \mathcal{X}} M_X)$\\
        $\phi^{\prime} \leftarrow \phi^{\prime} + \left\{(i, j) \mid \arg \max _{j^{\prime}} M_{i j^{\prime}}=j \wedge \arg \max _{i^{\prime}} M_{i^{\prime}j}=i\right\}$\\
        $\boldsymbol{H}_s, \boldsymbol{H}_t \leftarrow$ Relational-Encoder $\left(G_s, G_t, \phi^{\prime}\right)$\\
    }   
	return $M$ 
\end{algorithm}

